Leverage the Average: Averaged Sampling in Pre-Silicon Side-Channel Leakage Assessment

Pre-silicon side-channel leakage assessment is a useful tool to identify hardware vulnerabilities at design time, but it requires many high-resolution power traces and increases the power simulation cost of the design. By downsampling and averaging these high-resolution traces, we show that the power simulation cost can be considerably reduced without significant loss of side-channel leakage assessment quality. We introduce a theoretical basis for our claims. Our results demonstrate up to 6.5-fold power-simulation speed improvement on a gate-level side-channel leakage assessment of a RISC-V SoC. Furthermore, we clarify the conditions under which the averaged sampling technique can be successfully used.

==> sections/risc-v.tex <==
% RISC-V Assembler syntax and style for latex lstlisting package
% 
% These are risc-v commands as per our university (University Augsburg, Germany) guidelines.
%
% Author: Anton Lydike
%
% This code is in the public domain and free of licensing

% language definition
\lstdefinelanguage[RISC-V]{Assembler}
{
  alsoletter={.}, % allow dots in keywords
  alsodigit={0x}, % hex numbers are numbers too!
  morekeywords=[1]{ % instructions
    lb, lh, lw, lbu, lhu,
    sb, sh, sw,
    sll, slli, srl, srli, sra, srai,
    add, addi, sub, lui, auipc,
    xor, xori, or, ori, and, andi,
    slt, slti, sltu, sltiu,
    beq, bne, blt, bge, bltu, bgeu,
    j, jr, jal, jalr, ret,
    scall, break, nop
  },
  morekeywords=[2]{ % sections of our code and other directives
    .align, .ascii, .asciiz, .byte, .data, .double, .extern,
    .float, .globl, .half, .kdata, .ktext, .set, .space, .text, .word
  },
  morekeywords=[3]{ % registers
    zero, ra, sp, gp, tp, s0, fp,
    t0, t1, t2, t3, t4, t5, t6,
    s1, s2, s3, s4, s5, s6, s7, s8, s9, s10, s11,
    a0, a1, a2, a3, a4, a5, a6, a7,
    ft0, ft1, ft2, ft3, ft4, ft5, ft6, ft7,
    fs0, fs1, fs2, fs3, fs4, fs5, fs6, fs7, fs8, fs9, fs10, fs11,
    fa0, fa1, fa2, fa3, fa4, fa5, fa6, fa7
  },
  morecomment=[l]{;},   % mark ; as line comment start
  morecomment=[l]{\#},  % as well as # (even though it is unconventional)
  morestring=[b]",      % mark " as string start/end
  morestring=[b]'       % also mark ' as string start/end
}

% usage example:

% define some basic colors
\definecolor{mauve}{rgb}{0.58,0,0.82}

\lstset{
  % listings sonderzeichen (for german weirdness)
  literate={ö}{{\"o}}1
           {ä}{{\"a}}1
           {ü}{{\"u}}1,
  basicstyle=\tiny\ttfamily,                    % very small code
  breaklines=true,                              % break long lines
  commentstyle=\itshape\color{green!50!black},  % comments are green
  keywordstyle=[1]\color{blue!80!black},        % instructions are blue
  keywordstyle=[2]\color{orange!80!black},      % sections/other directives are orange
  keywordstyle=[3]\color{red!50!black},         % registers are red
  stringstyle=\color{mauve},                    % strings are from the telekom
  identifierstyle=\color{teal},                 % user declared addresses are teal
  frame=l,                                      % black line on the left side of code
  language=[RISC-V]Assembler,                   % all code is RISC-V
  tabsize=4,                                    % indent tabs with 4 spaces
  showstringspaces=false                        % do not replace spaces with weird underlines
}

==> sections/theory_long.tex <==
\section{Theoretical Background}
\label{sec:theory}

% - given that reducing the sample-rate is beneficial for simulation (saves us time with enough precision), how do we choose the sample-rate (and its corresponding power model)?

% three groups of signals in a netlist: 1. related to the secret value, 2. independent of the secret value but related to the controlled value, 3. independent of both the secret and controlled values. Group 1 will make correlation peaks higher and attack easier. Group 2 makes correlation lower and attack harder. Group 3 adds independent noise to the power traces (shouldn't affect the correlation much).
% Matlab simulated traces, averaging to reduce the horizontal noise, effect of collision of different secret bytes 

\subsection{Power Side-Channel Analysis}

\textbf{Problem Statement}
finding \textit{one} key byte

\textbf{DPA.}
Differential power analysis (DPA) \cite{kocher1999differential} reveals secret values (plaintext, key, ciphertext) based on a statistical method by comparing the means of two large sets of power traces. The higher the difference, the stronger the correlation. 

\textbf{CPA.}
Correlation power analysis (CPA) \cite{brier2004correlation} is a more advanced attack than DPA since it requires fewer traces and less computational time. CPA calculates the Pearson correlation coefficient between the actual power dissipation and the constructed leakage. A strong correlation happens when the coefficient is close to either -1 or 1.  

\textbf{Side-channel leakage assessment at design time} properties of an ideal power simulator\todo{simulation time vs #of samples}

% \textbf{Maximum Likelihood}

% leakage, key hypotheses, selection function, correlation
\todo{a road map to show the overall 3 cases: non-averaged, two averaged- synopsis table to summarize results}
\subsection{Non-Averaged Sampling}
In non-averaged sampling, each sample in the power trace can be broken into a part correlated to the select function $\zeta(x,k)$ and a select function-independent part stemming from other parts of the design (no measurement noise in simulated traces). 
We call the latter \textit{algorithmic noise}.
For N traces, each time sample $t_s$ in trace number n can be written as:
\begin{equation} \label{eq:smpl}
    P_{n,{t_s}} = \alpha . \zeta(x_n, k_{c_{t_s}}) + r_n + \mu_r
\end{equation} \todo{not Gaussian just zero-mean}
where $P_{n,{t_s}}$ denotes the power consumption at time sample $t_s$ of the $n^{th}$ power trace. $\alpha$ is an unknown constant. $\zeta(x_n, k_{c_{t_s}})$ is the select function dependent on the controllable variable in trace n ($x_n$) and the correct key in time sample $t_s$. We model the algorithmic noise as a zero-mean random noise 
% Gaussian distribution with mean 0 
% and standard deviation $\sigma$, \textit{i.e.}, $r_n \sim N(0, \sigma^2)$ 
and a constant unknown bias $\mu_r$.

Note that this model is similar to the model used by Fei et al. \cite{fei2014statistics}, however, we consider different time samples in the same trace can correlate with different correct key values. For instance, the SubBytes function in the AES algorithm working on different bytes of the key value in different time samples within the same trace. This notation is useful for our analyses in the rest of the paper. 

\textbf{Implications for DPA attack.}
Following the mentioned non-averaged sampling, we arrive at the following theorem.
\begin{theorem}
In non-averaged sampling, a sufficiently large number of power traces are required for a DPA attack to be successful.
\end{theorem}
\begin{proof}
Expanding the difference of means for the power consumption at time $t_s$ we have:
\begin{equation*}
    \begin{split}
        & \mathbb{E}(P_{n,{t_s}} \mid \zeta_n=1) - \mathbb{E}(P_{n,{t_s}} \mid \zeta_n=0) \\ 
        & = (\alpha + \mathbb{E}(r_n \mid \zeta_n=1) + \mu_r) - (\mathbb{E}(r_n \mid \zeta_n=0) + \mu_r) \\ 
        & = \alpha + \mathbb{E}(r_n \mid \zeta_n=1) - \mathbb{E}(r_n \mid \zeta_n=0) 
    \end{split}
\end{equation*}
where $\zeta_n$ is short for $\zeta(x_n,k_{c_{t_s}})$ and $\mathbb{E}(.)$ denotes the expectation function. \\
In general, $\mathbb{E}(r_n)$ terms might not cancel each other and as a result make the difference of means imprecise. However, for a sufficiently large number of traces, $\lim_{N\to\infty} (\mathbb{E}(r_n)) = 0$ therefore:
\begin{equation*}
    \begin{split}
        \mathbb{E}(P_{n,{t_s}} \mid \zeta_n=1) - \mathbb{E}(P_{n,{t_s}} \mid \zeta_n=0) & = \alpha
    \end{split}
\end{equation*}
which shows that the difference of means criteria is unaffected by the algorithmic noise.
\end{proof}


\textbf{Implications for CPA attack.} 
A similar theorem is reached for CPA attack on non-averaged traces.
\begin{theorem}
In non-averaged sampling, a sufficiently large number of power traces are required for a CPA attack to be successful.
\end{theorem}
\begin{proof}
The correlation coefficient between the select function with key guess and the power trace is the covariance between the two sets divided by their standard deviations:
\begin{equation*}
    \begin{split}
        \rho = \frac{\sum_{j=1}^{N} \left( \left( \Delta\zeta_{j,k_g} \right) \left( P_{j,t_s} - \overline{P_{t_s}} \right) \right) }{\sqrt{\sum_{j=1}^{N}\left( \Delta\zeta_{j,k_g} \right)^2 \sum_{j=1}^{N}\left( P_{j,t_s} - \overline{P_{t_s}} \right)^2}}
    \end{split}
\end{equation*}
where $k_g$ is the key guess, $k_{c_{t_s}}$ is the correct key at time sample $t_s$, 
\[\Delta\zeta_{j,k_g} = \zeta(x_j,k_g) - \overline{\zeta(x,k_g)},\]  
\[\overline{P_{t_s}} = \frac{\alpha}{N} \sum_{i=1}^{N} \zeta(x_i, k_{c_{t_s}}) + \frac{1}{N}\sum_{i=1}^{N}r_i + \mu_r.\] 
With enough traces, the average of random noise converges to zero and:  
\[\overline{P_{t_s}} = \frac{\alpha}{N} \sum_{i=1}^{N} \zeta(x_i, k_{c_{t_s}}) + \mu_r.\]
Therefore,
\[P_{j,t_s} - \overline{P_{t_s}} = \alpha.\Delta\zeta_{j,k_{c_{t_s}}} + r_j \]
where
\[\Delta\zeta_{j,k_{c_{t_s}}} = \zeta(x_j, k_{c_{t_s}}) - \frac{1}{N} \sum_{i=1}^{N}\zeta(x_i,k_{c_{t_s}}). \]
Because of the dependence of $P_{j,t_s}$ on random noise ($r_j$), the covariance term is imprecise and requires sufficiently large number of traces to converge. 
\end{proof}


\subsection{Averaged Sampling}
If a continuous-time model of the power consumption of a design is available, a power sample can be computed by averaging power consumption of certain time intervals. For instance, the power sample in the time interval ($t_{s_1},t_{s_2}$) in the $n^{th}$ power trace is:
% The power simulation tools like Cadence Joules report the \textit{average} power consumption of a design in the requested time intervals. Given that power simulation CAD tools work with a nearly-continuous-time power model, the power trace output of these tools for the given time interval ($t_{s_1}$, $t_{s_2}$) then can be written as:
\begin{equation} \label{eq:avg_smpl}
    \begin{split}
        P_{n,{t_{s_1},t_{s_2}}} & = avg(P_{n,{t_s}}) \mid_{t_s \in (t_{s_1},t_{s_2})} \\ 
        & = \frac{\alpha}{t_{s_2} - t_{s_1}} \int_{t_{s_1}}^{t_{s_2}} \zeta(x_n, k_{c_{\tau}}) \,d{\tau} \\
        & + \frac{1}{t_{s_2} - t_{s_1}} \int_{t_{s_1}}^{t_{s_2}} r_{n,{\tau}} \,d{\tau} + \mu_r .
    \end{split}
\end{equation}

The processed key values during the time interval ($t_{s_1}$, $t_{s_2}$) determine whether or not the averaged power samples will alleviate the PSCL detection. Hence, we separately analyze two scenarios in the following: 
\begin{enumerate}
    \item only one key value is processed during the time interval,
    \item multiple key values are processed during the time interval.
\end{enumerate}


\subsubsection{One key value during the time interval}
If the same key value ($k_{B_1}$) is processed during the interval ($t_{s_1}$, $t_{s_2}$), the power sample in this interval will be:
\begin{equation} \label{eq:avg_same_key_rand}
    P_{n,{t_{s_1},t_{s_2}}} & = \alpha \zeta(x_n, k_{B_1}) + \frac{1}{t_{s_2} - t_{s_1}} \int_{t_{s_1}}^{t_{s_2}} r_{n,{\tau}} \,d{\tau} + \mu_r .
\end{equation}

\begin{theorem}
With enough time samples processing the same key value, the averaged power samples are not affected by the algorithmic noise.
\end{theorem}
\begin{proof}
For a sufficiently long interval, we have:
\begin{equation*}
    \lim_{\Delta_{t_s} \to \infty}\int_{t_{s_1}}^{t_{s_1}+\Delta_{t_s}} r_{n,{\tau}} \,d{\tau} = 0.
\end{equation*}

In practice, if we have a long enough time interval correlating to one key value, \textit{i.e.}, $\Delta_{B_1} = t_{s_2} - t_{s_1} > \Delta_{thr}$, we have:
\begin{equation} \label{eq:avg_same_key}
    P_{n,{t_{B_1},t_{B_1}+\Delta_{B_1}}} \approx \alpha \zeta(x_n, k_{B_1}) + \mu_r .
\end{equation}
\end{proof}

\begin{definition}[constructive samples]
Since the power samples corresponding to the same key value being processed make the correlation between the power trace and the secret key value stronger by removing the algorithmic noise, we name them \textbf{\textit{constructive samples}}.

\end{definition}

\textbf{Implications for DPA attack.}
Assuming the averaged power samples we derive the next theorem.
\begin{theorem}
Given enough constructive samples in a power trace by design, DPA requires fewer traces to succeed using averaged sampling.
\end{theorem}
\begin{proof}
Depending on the design, if there are enough constructive samples to average out the random noise ($\Delta_{B_1} > \Delta_{thr}$), power samples will follow \autoref{eq:avg_same_key}. In this case, the difference of means criteria used in DPA requires much fewer traces to recover the key. \\
However, if the design does not provide sufficient constructive samples ($\Delta_{B_1} < \Delta_{thr}$), the power samples follow \autoref{eq:avg_same_key_rand} and difference of means is:
\begin{equation*}
    \begin{split}
        & \mathbb{E}(P_{n,{t_{s_1},t_{s_2}}} \mid \zeta_n=1) - \mathbb{E}(P_{n,{t_{s_1},t_{s_2}}} \mid \zeta_n=0) \\
        & = (\alpha + \frac{1}{t_{s_2}-t_{s_1}} \mathbb{E}(\int_{t_{s_1}}^{t_{s_2}} r_{n,{\tau}} \,d{\tau} \mid \zeta_n=1) + \mu_r) \\
        & - (\frac{1}{t_{s_2}-t_{s_1}} \mathbb{E}(\int_{t_{s_1}}^{t_{s_2}} r_{n,{\tau}} \,d{\tau} \mid \zeta_n=0) + \mu_r) \\
        & = \alpha + \frac{1}{t_{s_2}-t_{s_1}} \int_{t_{s_1}}^{t_{s_2}} \mathbb{E}(r_{n,{\tau}} \mid \zeta_n=1) - \mathbb{E}(r_{n,{\tau}} \mid \zeta_n=0) \,d{\tau} .
    \end{split}
\end{equation*}
where $\zeta_n$ is short for $\zeta(x_n,k_{B_1})$ and $\mathbb{E(.)}$ denotes the expectation function.
Therefore in order for DPA to be successful, a sufficiently large number of traces is required to bring the average of $r_n$ close to zero.
\end{proof}

\textbf{Implications for CPA attack.}
Assuming averaged sampling, a similar theorem can be derived for CPA attack.
\begin{theorem}
Given enough constructive samples in a power trace by design, CPA requires fewer traces to succeed using averaged sampling.
\end{theorem}
\begin{proof}
The correlation coefficient between the select function with key guess and the power trace is:
\begin{equation} \label{eq:rho_avg}
    \begin{split}
        \rho = \frac{\sum_{j=1}^{N} \left( \left( \Delta\zeta_{j,k_g} \right) \left( P_{j,t_{s_1},t_{s_2}} - \overline{P_{t_{s_1},t_{s_2}}} \right) \right) }{\sqrt{\sum_{j=1}^{N}\left( \Delta\zeta_{j,k_g} \right)^2 \sum_{j=1}^{N}\left( P_{j,t_{s_1},t_{s_2}} - \overline{P_{t_{s_1},t_{s_2}}} \right)^2}}    \end{split}
\end{equation}
Given there are enough constructive samples to be averaged in the interval ($t_{s_1},t_{s_2}$), we have:
\[ P_{j,t_{s_1},t_{s_2}} - \overline{P_{t_{s_1},t_{s_2}}} = \alpha.(\zeta(x_j,k_{B_1}) - \overline{\zeta(x,k_{B_1})} ) = \alpha.\Delta\zeta_{j,k_{B_1}}.\]
Therefore, the correlation is not affected by the algorithmic noise and CPA can converge with fewer traces. 

However, without enough constructive samples, we have:
\begin{equation*}
    \begin{split}
        P_{j,t_{s_1},t_{s_2}} - \overline{P_{t_{s_1},t_{s_2}}} & = \alpha .\Delta\zeta_{j, k_{B_1}} \\
        & + \frac{1}{t_{s_2} - t_{s_1}} \int_{t_{s_1}}^{t_{s_2}} (r_{j,{\tau}}-\overline{r_\tau}) \,d{\tau}.
    \end{split}
\end{equation*}
Therefore a sufficiently large number of traces is required for the random noise to reach its zero mean and render CPA successful.
\end{proof}

\subsubsection{Multiple key values during the time interval}
Wlog. we assume key value $k_{B_1}$ is processed in the first part of the interval ($t_{s_1}$, $t_{s_m}$) and other key values from the set $\overline{\{k_{B_1}\}}$ where ${k_{B_1} \not\in \overline{\{k_{B_1}\}}}$ are processed in the rest of the interval ($t_{s_m}$, $t_{s_2}$). 

% In this case, the power sample in the time interval ($t_{s_1}, t_{s_2}$) will be:
% \begin{equation*}
%     \begin{split}
%         P_{n,{t_{s_1},t_{s_2}}} = \alpha \zeta(x_n, k_{B_1}) & + \frac{\alpha}{t_{s_2}-t_{s_m}} \int_{t_{s_m}}^{t_{s_2}} \zeta(x_n, k_{\tau}) \,d\tau \\
%         & + \frac{1}{t_{s_2} - t_{s_1}} \int_{t_{s_1}}^{t_{s_2}} r_{n,{\tau}} \,d{\tau} + \mu_r .
%     \end{split}
% \end{equation*}
To further simplify our next analyses, we assume the time samples in interval ($t_{s_m}$, $t_{s_2}$) correspond to processing the same key value $k_{\overline{B_1}} \neq k_{B_1}$. Thus the power sample in interval ($t_{s_1}$, $t_{s_2}$) can be written as:
\begin{equation}\label{eq:avg_multikey}
    \begin{split}
        P_{n,{t_{s_1},t_{s_2}}} & = \alpha \zeta(x_n, k_{B_1}) + \alpha \zeta(x_n, k_{\overline{B_1}}) \\
        & + \frac{1}{t_{s_2} - t_{s_1}} \int_{t_{s_1}}^{t_{s_2}} r_{n,{\tau}} \,d{\tau} + \mu_r .
    \end{split}
\end{equation}

\textbf{Implications for DPA attack.}
Assuming more than one key value are processed in a power trace, we derive the next theorem.
\begin{theorem}
Averaging time samples corresponding to one key value with time samples corresponding with another key value diminishes the success probability of DPA attack even with a large number of power traces.
\end{theorem}
\begin{proof}
Following the simplified averaged sample in \autoref{eq:avg_multikey}, the difference of means used in DPA is:
\begin{equation*}
    \begin{split}
        & \mathbb{E}(P_{n,{t_{s_1},t_{s_2}}} \mid \zeta_n=1) - \mathbb{E}(P_{n,{t_{s_1},t_{s_2}}} \mid \zeta_n=0) \\
        & = (\alpha + \alpha \overline\zeta_n\mid_{\zeta_n=1} + \frac{1}{t_{s_2}-t_{s_1}} \mathbb{E}(\int_{t_{s_1}}^{t_{s_2}} r_{n,{\tau}} \,d{\tau} \mid \zeta_n=1) + \mu_r) \\
        & - (\alpha \overline\zeta_n\mid_{\zeta_n=0} + \frac{1}{t_{s_2}-t_{s_1}} \mathbb{E}(\int_{t_{s_1}}^{t_{s_2}} r_{n,{\tau}} \,d{\tau} \mid \zeta_n=0) + \mu_r) \\
        & = \alpha + \alpha (\overline\zeta_n\mid_{\zeta_n=1}-\overline\zeta_n\mid_{\zeta_n=0}) \\
        & + \frac{1}{t_{s_2}-t_{s_1}} \int_{t_{s_1}}^{t_{s_2}} \mathbb{E}(r_{n,{\tau}} \mid \zeta_n=1) - \mathbb{E}(r_{n,{\tau}} \mid \zeta_n=0) \,d{\tau}
    \end{split}
\end{equation*}
where $\zeta_n$ and $\overline\zeta_n$ are short for $\zeta(x_n,k_{B_1})$ and $\zeta(x_n,k_{\overline{B_1}})$ respectively.
Since $\overline\zeta_n\mid_{\zeta_n=1}$ and $\overline\zeta_n\mid_{\zeta_n=0}$ are not predictable, even with a sufficiently large number of traces for the random noise to reach its mean value of zero, still the DPA can be inconclusive.
\end{proof}


\textbf{Implications for CPA attack.}
A similar theorem is derived for CPA attack.
\begin{theorem}
Combining time samples corresponding to more than one key value diminishes the success probability of CPA attack even with a large number of power traces.
\end{theorem}
\begin{proof}
The correlation coefficient between the select function and the power trace is the same as in \autoref{eq:rho_avg}.
Similarly, following the simplified averaged sample in \autoref{eq:avg_multikey}, we have:
\begin{equation*}
    \begin{split}
        P_{j,t_{s_1},t_{s_2}} - \overline{P_{t_{s_1},t_{s_2}}} & = \alpha .\Delta\zeta_{j, k_{B_1}} + \alpha .\Delta\zeta_{j, k_\overline{{B_1}}}  \\
        & + \frac{1}{t_{s_2} - t_{s_1}} \int_{t_{s_1}}^{t_{s_2}} (r_{j,{\tau}}-\overline{r_\tau}) \,d{\tau}.
    \end{split}
\end{equation*}
Therefore, even with enough traces to cancel out the random noise, the term $\alpha .\Delta\zeta_{j, k_\overline{{B_1}}}$ greatly impairs the correlation.
\end{proof}
\textbf{Note.} Averaging power samples for $\kappa>1$ key values, compared to only one key value, will intrinsically make DPA and CPA harder to succeed. However, averaging power samples from $\kappa>2$ key values will not necessary make DPA and CPA results worse than averaging power samples from $\kappa'<\kappa, \kappa'\neq 1$ key values. \todo{refer to downsampled traces}

\begin{definition}[destructive samples]
Since the power samples corresponding to different key values being processed makes the correlation between the power trace and the secret key value weaker, we name them \textbf{\textit{destructive samples}}.
\end{definition}

\textbf{Simulated experiment setup.}
For our simulated experiments, we generate power traces in Matlab mimicking how real power traces are; Following the assumption that at each clock trigger, there is a rush of current in the circuit, we generate power traces in the shape of sawtooth function where the amplitude is a function of the current level and the period is similar to the system clock period. This model follows the so-called Delta-I noise \cite{gonzalez1999low} and is similar to the model used by Tiran et al. \cite{tiran2014model}.

SCA attacks like DPA and CPA exploit the dependency of the power consumption of a circuit on the secret data as well as a controlled data. To make our generated power traces applicable to such attacks, we further make the amplitude of the samples in each trace dependent on a function of a secret and a controlled byte. For our traces, we choose the function to be $f_{n,t_s} = xor(x_n, k_{t_s})$ where $x_n$ is the controlled value for the $n^{th}$ trace and $k_{t_s}$ is the secret value for the time sample $t_s$. \autoref{fig:matlab_trace} shows a generated power trace as an example for clock frequency of 80MHz. Each trace corresponds to one controlled value and contains 64 clock cycles. This is similar to measured traces in practice where an attacker feeds a device with known inputs and acquires one trace for each given input. Every 16 continuous clock cycles correspond to one key byte value. 

Note that these traces are interpolated in Matlab to work as a continuous-time power trace that we later sample or average to mimic power acquisition by oscilloscopes (non-averaged sampling) and power simulation by CAD tools (averaged sampling). This continuous-time model acts as the actual power consumption of a device (before being measured by an oscilloscope) and the internal model of power simulator before generating a power report for specific time intervals. We generate 256 such traces; One for each controlled data value. We use these traces for all of the simulated experiments in this section.
\begin{figure}
     \centering
     \begin{subfigure}
         \centering
         \includegraphics[width=\linewidth]{figures/IdealTrace1.pdf}
        %  \caption{$y=x$}
         \label{fig:matlab_ideal_trace}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}
         \centering
         \includegraphics[width=\linewidth]{figures/NoisyTrace1.pdf}
        %  \caption{$y=3sinx$}
         \label{fig:matlab_noisy_trace}
     \end{subfigure}
    %  \hfill
        \caption{Generated power traces using Matlab. Each trace processes 4 different key bytes. With each key byte taking 16 clock periods. Top: noise-less trace example. Bottom: noisy trace example with SANR=10.}
        \label{fig:matlab_trace}
\end{figure}

\textbf{Simulated experiment 1 - averaged vs. non-averaged sampling.}
From our 256 traces like the one shown in \autoref{fig:matlab_trace}, we generate noisy continuous-time traces with Signal-to-Algorithmic Noise Ratio (SANR)\footnote{We differentiate between the SNR pertaining to the measurement noise and the SNR pertaining to the algorithmic noise, calling the latter Signal-to-Algorithmic Noise Ratio (SANR).} values of \{10, 5, 1, 0.5, 0.25, 0.1\}.
For each SANR value we generate two different power traces:
\begin{enumerate}
    \item A non-averaged sampled version with a sampling frequency of 2$\times$ clock frequency. 
    \item An averaged sampled version with a sampling frequency of 2$\times$ clock frequency. 
\end{enumerate}
To generate the averaged power trace with sampling frequency of 2$\times$ the clock frequency, each clock cycle is divided into two equal intervals and the average of each interval is reported as the power sample.
We run CPA on the two sets of noisy traces for each key byte separately and calculate the rank of the correct key value. We repeat the same process of noisy trace generation, sampling, and CPA 100 times and report the average correct key rank in \autoref{fig:ave_vs_nonave}. 

As \autoref{fig:ave_vs_nonave} shows, the averaged rank of the correct key is 1 (successful attack) from SANR$>0.5$ and no more than 3 otherwise. However, the correct key rank for the non-averaged traces can be as high as 40 for our noisiest trace set (SANR$=0.1$) and gets close to 1 for SANR$>5$. This experiment shows the advantage of averaged sampling over non-averaged in power simulation.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/ave_vs_nonave.pdf}
    \caption{Correct key rank from CPA attack on 256 noisy traces with different SANR values for the four different key bytes. Solid (resp. dashed) lines show ranks for non-averaged (resp. averaged) sampled traces.}
    \label{fig:ave_vs_nonave}
\end{figure}\todo{change SNR to SANR in figure}

\textbf{Simulated experiment 2 - constructive samples.}
For the same set of power traces with SANR=0.1 (weakest SANR), we want to see the effect of averaging constructive samples. We keep averaging up to 16 clock cycles corresponding to the same key byte. As \autoref{fig:constructive} shows, the rank of the correct key value gets closer to one as more constructive samples are averaged, confirming Theorem 5.

\begin{figure}
    \centering
    \includegraphics[width=.9\linewidth]{figures/constructive.pdf}
    \caption{Impact of averaging constructive samples on rank of the correct key value for noisy traces with SANR=0.1. The ranks are averaged from 100 repetitions of the same experiment.}
    \label{fig:constructive}
\end{figure}


\textbf{Simulated experiment 3 - destructive samples.}
Similar to the previous experiment, this time we average 16 constructive clock cycles for each key byte and add up to 16 destructive clock cycles to the averaged sample to study the effect of destructive samples to CPA results. \autoref{fig:destructive} confirms the expected effect of destructive samples as the rank of the correct key value increases with higher destructive to constructive samples ratio attesting to Theorem 7. 

\begin{figure}
    \centering
    \includegraphics[width=.9\linewidth]{figures/destructive.pdf}
    \caption{Impact of averaging destructive samples on rank of the correct key value for noisy traces with SANR=0.1. The ranks are averaged from 100 repetitions of the same experiment.}
    \label{fig:destructive}
\end{figure}
